GaussHDR: High Dynamic Range Gaussian Splatting via Learning Unified 3D and 2D Local Tone Mapping

High dynamic range (HDR) novel view synthesis (NVS) aims to reconstruct HDR scenes by leveraging multi-view low dynamic range (LDR) images captured at different exposure levels. Current training paradigms with 3D tone mapping often result in unstable HDR reconstruction, while training with 2D tone mapping reduces the model's capacity to fit LDR images. Additionally, the global tone mapper used in existing methods can impede the learning of both HDR and LDR representations. To address these challenges, we present GaussHDR, which unifies 3D and 2D local tone mapping through 3D Gaussian splatting. Specifically, we design a residual local tone mapper for both 3D and 2D tone mapping that accepts an additional context feature as input. We then propose combining the dual LDR rendering results from both 3D and 2D local tone mapping at the loss level. Finally, recognizing that different scenes may exhibit varying balances between the dual results, we introduce uncertainty learning and use the uncertainties for adaptive modulation. Extensive experiments demonstrate that GaussHDR significantly outperforms state-of-the-art methods in both synthetic and real-world scenarios.

==> tables/ablation_sup.tex <==

\begin{table*}[htbp]
  \centering
  \caption{Ablation results on each component of the proposed GaussHDR. TM indicates tone mapping while Res. means the residual form of local tone mapper. All experiments are based on Scaffold-GS under the Exp-1 setting. All the metrics listed here represent PSNR.}
  \vspace{-2mm}
  \resizebox{0.85\textwidth}{!}{
    \begin{tabular}{c|c|c|cccccccccccc}
    \toprule
&\multirow{2}[4]{*}{Method} & \multirow{2}[4]{*}{LDR Test} & \multicolumn{2}{c}{HDR-NeRF~\cite{hdr-nerf} Real Scenes}                    & \multicolumn{3}{c}{HDR-NeRF~\cite{hdr-nerf} Synthetic Scenes} \\
\cmidrule(lr){4-5}\cmidrule(lr){6-8}        
& &       & LDR-OE & LDR-NE  & LDR-OE & LDR-NE & HDR \\
\midrule  
(a)&3D Global TM &  $I_{\text{3d}}$ &33.94 & 31.88& 42.03 & 40.44 & 26.11\\
(b) & 3D Local TM  &  $I_{\text{3d}}^*$ & 34.41 & 32.56 & 42.28 & 41.33 & 26.78\\
(c) & 2D Global TM &  $I_{\text{2d}}$ &32.45 &32.05 & 41.57 & 40.98& 37.96\\
(d) & 2D Local TM &  $I_{\text{2d}}^*$ & 34.19 & 32.92 & 41.95 & 41.34 & 38.35\\
(e)&  3D + 2D Global TM &  $I_{\text{merge}}$ & 33.22 & 32.80 & 41.73 & 41.23 & 38.27\\
(f)&3D + 2D Local TM &  $I_{\text{3d}}^*$ & 35.29 & 33.63 &42.44 & 41.58& \textbf{38.60}\\
(g)&3D + 2D Local TM &  $I_{\text{2d}}^*$ & 35.17 &	33.48 & 42.33 & 41.64& \textbf{38.60}\\
(h)&3D + 2D Local TM (w/o Res.)&  $I_{\text{merge}}$ & 35.08 & 32.63 & 42.78 & 41.73 & 18.46\\
(i)&\textbf{3D + 2D Local TM (Ours)} & $I_{\text{merge}}$ & \textbf{35.37} & \textbf{33.68} & \textbf{42.91} & \textbf{41.97} & \textbf{38.60} \\
    \bottomrule
    \end{tabular}}
    \vspace{-2mm}
  \label{tab:ablation}%
\end{table*}%




==> tables/hdrnerf-real-4.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Per-scene quantitative comparisons on HDR-NeRF~\cite{hdr-nerf} real datasets. LDR-OE and LDR-NE denote the LDR results with exposure $\{t_1,t_3,t_5\}$ and $\{t_2,t_4\}$, respectively. The training exposure setting is Exp-1.}
  \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{c|c|cccccccccccc}
    \toprule
&\multirow{2}[3]{*}{Method}  & \multicolumn{3}{c}{Box} & \multicolumn{3}{c}{Computer} & \multicolumn{3}{c}{Flower} & \multicolumn{3}{c}{Luckycat} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}    
&       & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ \\
\midrule  
 \multirow{5}[2]{*}{LDR-OE} & HDR-NeRF~\cite{hdr-nerf} & 31.54 & 0.953 & 0.068 & 32.42 &0.950 & 0.077 & 29.81 & 0.948 & 0.069 & 32.85 & 0.938 & 0.062\\
% & HDR-NeRF~\cite{hdr-nerf} $\dag$ & 31.78	& 0.958	& 0.062  & 32.55 &	0.945	& 0.079 & 30.76	& 0.952 &	0.059  & 32.70 &0.948	&0.063   \\
& HDR-GS~\cite{hdr-gs} $\dag$ & 34.39 &0.973&0.016  & 34.41 & 0.967 & 0.020 & 31.62 & 0.956 & 0.037 & 33.82 &0.961&0.022 \\
& \textbf{Ours (3DGS)} &  35.87  &  0.976&0.012 & 34.99 & 0.967 & 0.020 & 31.84 & 0.958 & 0.024 & 34.03 & 0.961 & 0.020\\
& HDR-Scaffold-GS~\cite{scaf-gs} $*$ & 34.66  &  0.974 & 0.012 & 34.55 &0.965&0.017& 32.70 & 0.967&0.019 &34.43&0.963&0.016\\
& \textbf{Ours (Scaffold-GS)} &  \textbf{36.24} & \textbf{0.979} & \textbf{0.010} & \textbf{35.50} & \textbf{0.970} & \textbf{0.015} & \textbf{34.12} & \textbf{0.971} & \textbf{0.014} &\textbf{35.61} &\textbf{0.970}&\textbf{0.015}  \\    
\midrule     
 \multirow{5}[2]{*}{LDR-NE} & HDR-NeRF~\cite{hdr-nerf} &31.40&
0.944 & 0.079  & 31.21 & 0.931 & 0.098 & 30.05 & 0.949 &0.058 &
33.13 & 0.948 & 0.051  \\
% & HDR-NeRF~\cite{hdr-nerf} $\dag$ & 31.25 &	0.957 & 0.062  & 32.61	& 0.947&	0.081  & 30.45	&0.951&	0.062 &32.70	& 0.944&	0.062   \\
& HDR-GS~\cite{hdr-gs} $\dag$ & 30.17 & 0.967 & 0.021 &32.78 & 0.966 & 0.023 & 30.21 & 0.954 & 0.039 & 31.55 &0.954 & 0.026\\
& \textbf{Ours (3DGS)} &  32.57  &0.972& 0.014 & 34.18 &0.966 & 0.022 & 30.52 & 0.956 & 0.027 & 33.24 & 0.956 & 0.022\\
& HDR-Scaffold-GS~\cite{scaf-gs} $*$ & 31.87  &   0.970 & 0.015&33.16&0.964&0.019 &30.68 & 0.964 &0.021&31.80&0.957&0.019 \\
& \textbf{Ours (Scaffold-GS)} & \textbf{32.93} & \textbf{0.974} & \textbf{0.013}  & \textbf{34.95} & \textbf{0.968} & \textbf{0.017} & \textbf{32.35} & \textbf{0.970} & \textbf{0.016} &\textbf{34.48}&\textbf{0.965}&\textbf{0.016}  \\    
    \bottomrule
    \end{tabular}}
       \begin{tablenotes}
        \footnotesize
        \item $\dag$ We re-implement HDR-GS~\cite{hdr-gs} under Exp-1 setting for fair comparison.
        \item $*$ We replace the scene representation in HDR-GS from 3DGS~\cite{3dgs} to Scaffold-GS~\cite{scaf-gs} to establish a baseline for our method utilizing Scaffold-GS.
     \end{tablenotes}
  \label{tab:hdrnerf-real-4}%
\end{table*}%



% \begin{table*}[th]
%     \small
%     \centering
%     \caption{Quantitative comparisons with baseline methods on synthetic and real scenes. Metrics are averaged over the scenes from our dataset (per-scene metrics are shown in supplementary material). LDR-OE denotes the LDR results with exposure $t_1$, $t_3$, and $t_5$. LDR-NE denotes the LDR results with exposure $t_2$, and $t_4$. HDR denotes the HDR results. We color code each column as \colorbox{best}{best} and \colorbox{second}{second best}.}
    
%     \begin{threeparttable}
%     \begin{tabular}{@{}p{60pt}|p{30pt}|p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering}}
%     % \begin{tabularx}{\textwidth}{lCCCCCCCCCCCCC}
%         \hline 
%         % \toprule
%         & & \multicolumn{3}{c}{LDR-OE ($t_1,t_3,t_5$)} 
%         & \multicolumn{3}{c}{LDR-NE ($t_2,t_4$)}
%         & \multicolumn{3}{c}{HDR} \\
%         % \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
%         \cline{3-11} 
%     &   & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
%         \hline
%         % \midrule

% % NeRF-W\cite{martin2021nerf}      & 28.55   & 0.927   & 0.094  & 28.64   & 0.923   & 0.089\\
% % Ours$\dag$   & 30.37   & 0.944   & 0.075 & 29.37   & 0.938   & 0.078 \\
% % Ours        & 31.63   & 0.948   & 0.069  & 31.43   & 0.943   & 0.069\\
% % NeRF-GT\cite{mildenhall2020nerf}    & 34.55   & 0.958   & 0.057   & 34.59   & 0.956   & 0.051\\

% \multirow{2}*{NeRF\cite{mildenhall2020nerf}} 
% & Syn.  & 13.97 	& 0.555  &0.376 & ---  & ---  & ---  & --- & --- & --- \\ 
% & Real  & 14.95   & 0.661   & 0.308  & ---     & ---     &  ---      &  ---      & ---   &  ---    \\

%         \hline
%         % \midrule
% \multirow{2}*{NeRF-W\tnote{1} \cite{martin2021nerf}} 
% & Syn.  & 29.83 	& 0.936  & 0.047  & 29.22 	& 0.927 	& 0.050 
% & ---  & ---   & ---   \\
% & Real  & 28.55   & 0.927   & 0.094  & 28.64   & 0.923   & 0.089  & --- & --- & ---  \\
%         \hline
%         % \midrule
% \multirow{2}*{NeRF-GT\tnote{2} \cite{mildenhall2020nerf}} 
% & Syn.  &\cellcolor{second}37.66   &\cellcolor{second}0.965   &\cellcolor{second}0.028    &\cellcolor{second}35.87  &\cellcolor{second}0.955   &\cellcolor{second}0.032  &\cellcolor{best}37.80 &\cellcolor{best}0.964  &\cellcolor{best}0.029 \\
% & Real  &\cellcolor{best}34.55   &\cellcolor{best}0.958   &\cellcolor{best}0.057   &\cellcolor{best}34.59   &\cellcolor{best}0.956   &\cellcolor{best}0.051  & --- & --- & ---   \\
% \hline
% \multirow{2}*{Ours$\dag$}  
% & Syn.  & ---   & ---   & --- & ---   & ---  & ---  & --- & --- & ---   \\
% & Real  & 30.37   & 0.944   & 0.075 & 29.37   & 0.938   & 0.078  & --- & --- & ---   \\

% \hline
% \multirow{2}*{Ours} 
% & Syn.  &\cellcolor{best}39.07 &\cellcolor{best}0.973 &\cellcolor{best}0.026 &\cellcolor{best}37.53 &\cellcolor{best}0.966 &\cellcolor{best}0.024 &\cellcolor{second}36.40 &\cellcolor{second}0.936 &\cellcolor{second}0.018 \\
% & Real  & \cellcolor{second}31.63   & \cellcolor{second}0.948   & \cellcolor{second}0.069  & \cellcolor{second}31.43   & \cellcolor{second}0.943   & \cellcolor{second}0.069  & --- & --- & ---   \\
% \hline
%     \end{tabular}
%     \begin{tablenotes}
%         \footnotesize
%         \item[1] The exposures of input views for NeRF-W are randomly selected from all five exposures to learn five appearance vectors for testing.
%         \item[2] A  version of  NeRF (as the upper bound of our method) that  is  trained  from  LDR  images  with  consistent exposures or HDR images.
%         \item[$\dag$] An ablation study of our method that models the tone-mapping operations of RGB channels with a single MLP.
%      \end{tablenotes}
%     \end{threeparttable}
%     \label{tb:cmp_syn}
    
% \end{table*}

==> tables/hdrnerf-syn-8-1.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Per-scene quantitative comparisons on HDR-NeRF~\cite{hdr-nerf} synthetic datasets (Part 1). LDR-OE and LDR-NE denote the LDR results with exposure $\{t_1,t_3,t_5\}$ and $\{t_2,t_4\}$, respectively. HDR denotes the HDR results. The training exposure setting is Exp-1.}
  \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{c|c|cccccccccccc}
    \toprule
&\multirow{2}[3]{*}{Method}  & \multicolumn{3}{c}{Bathroom} & \multicolumn{3}{c}{Bear} & \multicolumn{3}{c}{Chair} & \multicolumn{3}{c}{Diningroom} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}    
&       & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ \\
\midrule  
 \multirow{5}[2]{*}{LDR-OE} & HDR-NeRF~\cite{hdr-nerf} &36.26 &0.949 &0.037  & 42.91 &0.990 & 0.010 &32.45&0.905&0.081&41.23&0.986&0.010   \\
% & HDR-NeRF~\cite{hdr-nerf} $\dag$ &36.83  & 0.944 & 0.037  &   43.13& 0.990& 0.008 &  34.63& 0.933& 0.058&43.47& 0.988& 0.008   \\
& HDR-GS~\cite{hdr-gs} $\dag$ &   38.06     & 0.963      &   0.020  &41.61	&0.989	&0.005  &35.07	&0.952&	0.024 & 38.26&	0.979&	0.014 \\
& \textbf{Ours (3DGS)} & 41.12& 0.975&	0.008&44.44 &	0.992&	0.003 & 37.05 &	0.968&	0.014 &39.63&0.981	&0.017  \\
& HDR-Scaffold-GS~\cite{scaf-gs} $*$ &  41.21 &	0.977&	0.008 &44.56&	0.992&	0.003 &36.36 &	0.966&	0.016 &44.87&	\textbf{0.994}	&\textbf{0.002}  \\
& \textbf{Ours (Scaffold-GS)} & \textbf{42.08}&	\textbf{0.981}&	\textbf{0.006}    &\textbf{45.40} &\textbf{0.993}	&\textbf{0.002}  &\textbf{37.65}&\textbf{0.971}&	\textbf{0.012}& \textbf{45.21}	&\textbf{0.994}	&\textbf{0.002}     \\    
\midrule     
 \multirow{5}[2]{*}{LDR-NE} & HDR-NeRF~\cite{hdr-nerf} &33.44&0.926&0.046&41.19&0.987&0.012&30.78&0.886&0.083&37.99&0.979&0.013       \\
% & HDR-NeRF~\cite{hdr-nerf} $\dag$ &  36.30     &  0.945  & 0.039 & 42.13& 0.989& 0.009   &  34.10& 0.929 &0.064 &39.81 &0.983&0.011  \\
& HDR-GS~\cite{hdr-gs} $\dag$ &  36.03	&0.963 &	0.024  & 41.69	&0.988	&0.005 &34.05 & 0.951	&0.026&34.62&	0.976&	0.020 \\
& \textbf{Ours (3DGS)} &  41.10&	0.977	&0.008&43.85 &0.992&	0.003 & 36.53&0.967	&0.015&38.78&0.980&0.021 \\
& HDR-Scaffold-GS~\cite{scaf-gs} $*$ &  40.61	&0.979	&0.008 &42.10	&0.992	&0.004 & 35.89&0.965&	0.017 & 41.00	&\textbf{0.993}	&\textbf{0.003}  \\
& \textbf{Ours (Scaffold-GS)} & \textbf{41.71} &	\textbf{0.982}&	\textbf{0.007}&\textbf{44.43} & \textbf{0.993}	&\textbf{0.002} &\textbf{37.14}&	\textbf{0.970}	&\textbf{0.013} &\textbf{43.33}&	\textbf{0.993}&	\textbf{0.003} \\    
\midrule
 \multirow{5}[2]{*}{HDR} & HDR-NeRF~\cite{hdr-nerf} &33.97&0.925&0.048&\textbf{43.22}&\textbf{0.991}&0.008&34.14&0.924&0.069&38.57&0.981&0.015     \\
% & HDR-NeRF~\cite{hdr-nerf} $\dag$ &  33.80& 0.921&0.050& 42.66 &0.990&0.008  & 31.82& 0.920&0.083     \\
& HDR-GS~\cite{hdr-gs} $\dag$ &  15.48	&0.739&	0.125 &30.99	&0.961 &0.027&20.47	&0.751	&0.115 &18.86&0.860&0.074 \\
& \textbf{Ours (3DGS)} &  34.87	&0.943&	0.024 &41.47&	0.987	&0.007 &36.75&0.961	&0.019 & 34.82	&0.967	&0.028 \\
& HDR-Scaffold-GS~\cite{scaf-gs} $*$ &  22.28	&0.873	&0.061  &29.79	&0.970&	0.021&24.27&0.842&	0.163&26.60&0.952	&0.037  \\
& \textbf{Ours (Scaffold-GS)} &\textbf{36.22}	&\textbf{0.952}&	\textbf{0.017} & 42.23 & 0.988&	\textbf{0.005}& \textbf{37.79}&	\textbf{0.966}	&\textbf{0.017}&\textbf{38.61}&\textbf{0.983}	&\textbf{0.007}\\  
    \bottomrule
    \end{tabular}}
       \begin{tablenotes}
        \footnotesize
        \item $\dag$ We re-implement HDR-GS~\cite{hdr-gs} under Exp-1 setting for fair comparison.
        \item $*$ We replace the scene representation in HDR-GS from 3DGS~\cite{3dgs} to Scaffold-GS~\cite{scaf-gs} to establish a baseline for our method utilizing Scaffold-GS.
     \end{tablenotes}
  \label{tab:addlabel}%
\end{table*}%



% \begin{table*}[th]
%     \small
%     \centering
%     \caption{Quantitative comparisons with baseline methods on synthetic and real scenes. Metrics are averaged over the scenes from our dataset (per-scene metrics are shown in supplementary material). LDR-OE denotes the LDR results with exposure $t_1$, $t_3$, and $t_5$. LDR-NE denotes the LDR results with exposure $t_2$, and $t_4$. HDR denotes the HDR results. We color code each column as \colorbox{best}{best} and \colorbox{second}{second best}.}
    
%     \begin{threeparttable}
%     \begin{tabular}{@{}p{60pt}|p{30pt}|p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering}}
%     % \begin{tabularx}{\textwidth}{lCCCCCCCCCCCCC}
%         \hline 
%         % \toprule
%         & & \multicolumn{3}{c}{LDR-OE ($t_1,t_3,t_5$)} 
%         & \multicolumn{3}{c}{LDR-NE ($t_2,t_4$)}
%         & \multicolumn{3}{c}{HDR} \\
%         % \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
%         \cline{3-11} 
%     &   & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
%         \hline
%         % \midrule

% % NeRF-W\cite{martin2021nerf}      & 28.55   & 0.927   & 0.094  & 28.64   & 0.923   & 0.089\\
% % Ours$\dag$   & 30.37   & 0.944   & 0.075 & 29.37   & 0.938   & 0.078 \\
% % Ours        & 31.63   & 0.948   & 0.069  & 31.43   & 0.943   & 0.069\\
% % NeRF-GT\cite{mildenhall2020nerf}    & 34.55   & 0.958   & 0.057   & 34.59   & 0.956   & 0.051\\

% \multirow{2}*{NeRF\cite{mildenhall2020nerf}} 
% & Syn.  & 13.97 	& 0.555  &0.376 & ---  & ---  & ---  & --- & --- & --- \\ 
% & Real  & 14.95   & 0.661   & 0.308  & ---     & ---     &  ---      &  ---      & ---   &  ---    \\

%         \hline
%         % \midrule
% \multirow{2}*{NeRF-W\tnote{1} \cite{martin2021nerf}} 
% & Syn.  & 29.83 	& 0.936  & 0.047  & 29.22 	& 0.927 	& 0.050 
% & ---  & ---   & ---   \\
% & Real  & 28.55   & 0.927   & 0.094  & 28.64   & 0.923   & 0.089  & --- & --- & ---  \\
%         \hline
%         % \midrule
% \multirow{2}*{NeRF-GT\tnote{2} \cite{mildenhall2020nerf}} 
% & Syn.  &\cellcolor{second}37.66   &\cellcolor{second}0.965   &\cellcolor{second}0.028    &\cellcolor{second}35.87  &\cellcolor{second}0.955   &\cellcolor{second}0.032  &\cellcolor{best}37.80 &\cellcolor{best}0.964  &\cellcolor{best}0.029 \\
% & Real  &\cellcolor{best}34.55   &\cellcolor{best}0.958   &\cellcolor{best}0.057   &\cellcolor{best}34.59   &\cellcolor{best}0.956   &\cellcolor{best}0.051  & --- & --- & ---   \\
% \hline
% \multirow{2}*{Ours$\dag$}  
% & Syn.  & ---   & ---   & --- & ---   & ---  & ---  & --- & --- & ---   \\
% & Real  & 30.37   & 0.944   & 0.075 & 29.37   & 0.938   & 0.078  & --- & --- & ---   \\

% \hline
% \multirow{2}*{Ours} 
% & Syn.  &\cellcolor{best}39.07 &\cellcolor{best}0.973 &\cellcolor{best}0.026 &\cellcolor{best}37.53 &\cellcolor{best}0.966 &\cellcolor{best}0.024 &\cellcolor{second}36.40 &\cellcolor{second}0.936 &\cellcolor{second}0.018 \\
% & Real  & \cellcolor{second}31.63   & \cellcolor{second}0.948   & \cellcolor{second}0.069  & \cellcolor{second}31.43   & \cellcolor{second}0.943   & \cellcolor{second}0.069  & --- & --- & ---   \\
% \hline
%     \end{tabular}
%     \begin{tablenotes}
%         \footnotesize
%         \item[1] The exposures of input views for NeRF-W are randomly selected from all five exposures to learn five appearance vectors for testing.
%         \item[2] A  version of  NeRF (as the upper bound of our method) that  is  trained  from  LDR  images  with  consistent exposures or HDR images.
%         \item[$\dag$] An ablation study of our method that models the tone-mapping operations of RGB channels with a single MLP.
%      \end{tablenotes}
%     \end{threeparttable}
%     \label{tb:cmp_syn}
    
% \end{table*}

==> tables/hdrnerf-syn-8-2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Per-scene quantitative comparisons on HDR-NeRF~\cite{hdr-nerf} synthetic datasets (Part 2). LDR-OE and LDR-NE denote the LDR results with exposure $\{t_1,t_3,t_5\}$ and $\{t_2,t_4\}$, respectively. HDR denotes the HDR results. The training exposure setting is Exp-1.}
  \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{c|c|cccccccccccc}
    \toprule
&\multirow{2}[3]{*}{Method}  & \multicolumn{3}{c}{Dog} & \multicolumn{3}{c}{Desk} & \multicolumn{3}{c}{Sofa} & \multicolumn{3}{c}{Sponza} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}    
&       & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ \\
\midrule  
 \multirow{5}[2]{*}{LDR-OE} & HDR-NeRF~\cite{hdr-nerf} &37.77&0.981&0.016&  37.84&0.972&0.023 & 38.29&0.977&0.014 &  34.49&0.958&0.034     \\
% & HDR-NeRF~\cite{hdr-nerf} $\dag$ &       &       &       &       &       &       &       &       &       &       &       &        \\
& HDR-GS~\cite{hdr-gs} $\dag$ & 42.28 &	0.991	&0.004&39.81 &0.980	&0.007 & 41.75&0.989&0.004&37.99&0.972&0.016    \\
& \textbf{Ours (3DGS)} &43.06&	0.992&	0.004&42.28 &0.987&	0.004&43.04&0.990&\textbf{0.003}&41.43&0.986&0.007\\
& HDR-Scaffold-GS~\cite{scaf-gs} $*$ &  43.31&	0.993&	0.003 & 41.72 &	0.987&0.004 &43.26&\textbf{0.992}&\textbf{0.003} &42.43&0.990&\textbf{0.004} \\
& \textbf{Ours (Scaffold-GS)} & \textbf{43.76} &	\textbf{0.994}	&\textbf{0.002}   &\textbf{43.04}&	\textbf{0.990} &	\textbf{0.003} &\textbf{43.44} &	\textbf{0.992}	&\textbf{0.003} &\textbf{42.91}	&\textbf{0.991}&\textbf{0.004}  \\    
\midrule     
 \multirow{5}[2]{*}{LDR-NE} & HDR-NeRF~\cite{hdr-nerf} &36.52&0.976&0.018&35.26&0.960&0.029&38.35&0.976&0.014 &33.41&0.950&0.038 \\
% & HDR-NeRF~\cite{hdr-nerf} $\dag$ &       &       &       &       &       &       &       &       &       &       &       &        \\
& HDR-GS~\cite{hdr-gs} $\dag$ & 40.66 &	0.990&0.004  &38.47&	0.980&	0.007&41.55 & 0.989	&0.004 &36.99&0.975&0.015  \\
& \textbf{Ours (3DGS)} &  \textbf{42.24} &	0.991&	0.004  & 42.12 &	0.987	&0.004 & \textbf{42.34}&0.991&\textbf{0.003}&41.25&0.988&0.006 \\
& HDR-Scaffold-GS~\cite{scaf-gs} $*$ &  40.52 &	0.992&	0.004 &40.46&0.987	&0.004 &41.91&0.991&0.004 &41.02&0.990&0.004 \\
& \textbf{Ours (Scaffold-GS)} &  42.12 &	\textbf{0.993}	& \textbf{0.003}  &\textbf{42.76}&	\textbf{0.989}	&\textbf{0.003} &42.03&\textbf{0.992}	&\textbf{0.003}&\textbf{42.60}&\textbf{0.992}&\textbf{0.003} \\    
\midrule
 \multirow{5}[2]{*}{HDR} & HDR-NeRF~\cite{hdr-nerf} &\textbf{37.72}&\textbf{0.980}&0.016&43.38&\textbf{0.993}&0.007&\textbf{39.05}&\textbf{0.976}&0.017 &32.33&0.939&0.049   \\
% & HDR-NeRF~\cite{hdr-nerf} $\dag$ &       &       &       &       &       &       &       &       &       &       &       &        \\
& HDR-GS~\cite{hdr-gs} $\dag$ & 23.02 &	0.926&	0.037&29.11&0.773&0.082&26.60&0.928	&0.046&16.12&0.782&0.095  \\
& \textbf{Ours (3DGS)} &   36.36 &	0.973	& 0.016 &\textbf{43.98} &\textbf{0.993}&	0.006 &36.70&0.966&0.016 &34.32&0.964&0.023 \\
& HDR-Scaffold-GS~\cite{scaf-gs} $*$ &  24.33&	0.934&	0.040 &31.40&0.929&	0.044 &28.42&0.947&0.032&21.81&0.870&0.095   \\
& \textbf{Ours (Scaffold-GS)} &  37.52 &	0.978&	\textbf{0.012}  &43.83&\textbf{0.993}&\textbf{0.005} &36.99&0.969&\textbf{0.013} &\textbf{35.64}&\textbf{0.972}&\textbf{0.014}  \\  
    \bottomrule
    \end{tabular}}
       \begin{tablenotes}
        \footnotesize
        \item $\dag$ We re-implement HDR-GS~\cite{hdr-gs} under Exp-1 setting for fair comparison.
        \item $*$ We replace the scene representation in HDR-GS from 3DGS~\cite{3dgs} to Scaffold-GS~\cite{scaf-gs} to establish a baseline for our method utilizing Scaffold-GS.
     \end{tablenotes}
  \label{tab:addlabel}%
\end{table*}%



==> tables/hdrplenoxels-real-4.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Per-scene quantitative comparisons on HDR-Plenoxels~\cite{hdr-plenoxels} real datasets. LDR-OE and LDR-NE denote the LDR results with exposure $\{t_1,t_3,t_5\}$ and $\{t_2,t_4\}$, respectively. The training exposure setting is Exp-1.}
  \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{c|c|cccccccccccc}
    \toprule
&\multirow{2}[3]{*}{Method}  & \multicolumn{3}{c}{Character} & \multicolumn{3}{c}{Coffee} & \multicolumn{3}{c}{Desk} & \multicolumn{3}{c}{Plant} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}    
&       & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ \\
\midrule  
 \multirow{4}[1]{*}{LDR-OE} & HDR-GS~\cite{hdr-gs} $\dag$ & 34.96 & 0.978 &0.027 &27.79 & 0.943 &  0.049 & 28.78 & 0.922 &0.045& 29.18 & 0.930 & 0.054\\
& \textbf{Ours (3DGS)} &    36.73   & 0.980 & 0.025 & 28.35 & 0.947 & 0.046 &29.14 & 0.925 & 0.041 & 29.76 & 0.934 & 0.051 \\
& HDR-Scaffold-GS~\cite{scaf-gs} $*$ & 36.81  &0.979&0.029 & 28.31 & 0.946 & 0.043 & 28.64 & 0.919 & 0.049 & 30.44 & 0.930 & 0.059 \\
& \textbf{Ours (Scaffold-GS)} &  \textbf{38.24} & \textbf{0.983} & \textbf{0.018} &\textbf{29.31} & \textbf{0.955} & \textbf{0.032} & \textbf{29.91} & \textbf{0.933} & \textbf{0.035} & \textbf{31.48} & \textbf{0.945} & \textbf{0.040}   \\    
\midrule     
 \multirow{4}[1]{*}{LDR-NE} & HDR-GS~\cite{hdr-gs} $\dag$ & - & - &- &- &- &- & 27.08 &0.912 & 0.050 & 28.17 & 0.920 & 0.061  \\
& \textbf{Ours (3DGS)} &  - & - &- &- &- &- & 27.30 & 0.917 & 0.044 & 28.85 & 0.929 & 0.055 \\
& HDR-Scaffold-GS~\cite{scaf-gs} $*$ & - & - &- &- &- &-  & 27.03 & 0.911 & 0.053 & 29.23 & 0.920 &  0.065    \\
& \textbf{Ours (Scaffold-GS)} & - & - &- &- &- &-  &  \textbf{27.41} & \textbf{0.922} & \textbf{0.038}  & \textbf{30.55} & \textbf{0.941} & \textbf{0.044}      \\  
    \bottomrule
    \end{tabular}}
       \begin{tablenotes}
        \footnotesize
        \item $\dag$ We re-implement HDR-GS~\cite{hdr-gs} under Exp-1 setting for fair comparison.
        \item $*$ We replace the scene representation in HDR-GS from 3DGS~\cite{3dgs} to Scaffold-GS~\cite{scaf-gs} to establish a baseline for our method utilizing Scaffold-GS.
     \end{tablenotes}
  \label{tab:addlabel}%
\end{table*}%



% \begin{table*}[th]
%     \small
%     \centering
%     \caption{Quantitative comparisons with baseline methods on synthetic and real scenes. Metrics are averaged over the scenes from our dataset (per-scene metrics are shown in supplementary material). LDR-OE denotes the LDR results with exposure $t_1$, $t_3$, and $t_5$. LDR-NE denotes the LDR results with exposure $t_2$, and $t_4$. HDR denotes the HDR results. We color code each column as \colorbox{best}{best} and \colorbox{second}{second best}.}
    
%     \begin{threeparttable}
%     \begin{tabular}{@{}p{60pt}|p{30pt}|p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering} p{30pt}<{\centering}}
%     % \begin{tabularx}{\textwidth}{lCCCCCCCCCCCCC}
%         \hline 
%         % \toprule
%         & & \multicolumn{3}{c}{LDR-OE ($t_1,t_3,t_5$)} 
%         & \multicolumn{3}{c}{LDR-NE ($t_2,t_4$)}
%         & \multicolumn{3}{c}{HDR} \\
%         % \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
%         \cline{3-11} 
%     &   & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
%         \hline
%         % \midrule

% % NeRF-W\cite{martin2021nerf}      & 28.55   & 0.927   & 0.094  & 28.64   & 0.923   & 0.089\\
% % Ours$\dag$   & 30.37   & 0.944   & 0.075 & 29.37   & 0.938   & 0.078 \\
% % Ours        & 31.63   & 0.948   & 0.069  & 31.43   & 0.943   & 0.069\\
% % NeRF-GT\cite{mildenhall2020nerf}    & 34.55   & 0.958   & 0.057   & 34.59   & 0.956   & 0.051\\

% \multirow{2}*{NeRF\cite{mildenhall2020nerf}} 
% & Syn.  & 13.97 	& 0.555  &0.376 & ---  & ---  & ---  & --- & --- & --- \\ 
% & Real  & 14.95   & 0.661   & 0.308  & ---     & ---     &  ---      &  ---      & ---   &  ---    \\

%         \hline
%         % \midrule
% \multirow{2}*{NeRF-W\tnote{1} \cite{martin2021nerf}} 
% & Syn.  & 29.83 	& 0.936  & 0.047  & 29.22 	& 0.927 	& 0.050 
% & ---  & ---   & ---   \\
% & Real  & 28.55   & 0.927   & 0.094  & 28.64   & 0.923   & 0.089  & --- & --- & ---  \\
%         \hline
%         % \midrule
% \multirow{2}*{NeRF-GT\tnote{2} \cite{mildenhall2020nerf}} 
% & Syn.  &\cellcolor{second}37.66   &\cellcolor{second}0.965   &\cellcolor{second}0.028    &\cellcolor{second}35.87  &\cellcolor{second}0.955   &\cellcolor{second}0.032  &\cellcolor{best}37.80 &\cellcolor{best}0.964  &\cellcolor{best}0.029 \\
% & Real  &\cellcolor{best}34.55   &\cellcolor{best}0.958   &\cellcolor{best}0.057   &\cellcolor{best}34.59   &\cellcolor{best}0.956   &\cellcolor{best}0.051  & --- & --- & ---   \\
% \hline
% \multirow{2}*{Ours$\dag$}  
% & Syn.  & ---   & ---   & --- & ---   & ---  & ---  & --- & --- & ---   \\
% & Real  & 30.37   & 0.944   & 0.075 & 29.37   & 0.938   & 0.078  & --- & --- & ---   \\

% \hline
% \multirow{2}*{Ours} 
% & Syn.  &\cellcolor{best}39.07 &\cellcolor{best}0.973 &\cellcolor{best}0.026 &\cellcolor{best}37.53 &\cellcolor{best}0.966 &\cellcolor{best}0.024 &\cellcolor{second}36.40 &\cellcolor{second}0.936 &\cellcolor{second}0.018 \\
% & Real  & \cellcolor{second}31.63   & \cellcolor{second}0.948   & \cellcolor{second}0.069  & \cellcolor{second}31.43   & \cellcolor{second}0.943   & \cellcolor{second}0.069  & --- & --- & ---   \\
% \hline
%     \end{tabular}
%     \begin{tablenotes}
%         \footnotesize
%         \item[1] The exposures of input views for NeRF-W are randomly selected from all five exposures to learn five appearance vectors for testing.
%         \item[2] A  version of  NeRF (as the upper bound of our method) that  is  trained  from  LDR  images  with  consistent exposures or HDR images.
%         \item[$\dag$] An ablation study of our method that models the tone-mapping operations of RGB channels with a single MLP.
%      \end{tablenotes}
%     \end{threeparttable}
%     \label{tb:cmp_syn}
    
% \end{table*}

==> tables/sup_table1.tex <==
\begin{table*}[h]
  \centering
  % \vspace{-180mm}
  \caption{Quantitative comparisons on HDR-NeRF~\cite{hdr-nerf} and HDR-Plenoxels~\cite{hdr-plenoxels} real datasets. Metrics are averaged over all scenes. LDR-OE and LDR-NE denote the LDR results with exposure $\{t_1,t_3,t_5\}$ and $\{t_2,t_4\}$, respectively. The training exposure setting is Exp-1.}
  \vspace{-2mm}
  \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{c|cccccccccccc}
    \toprule
\multirow{3}[4]{*}{Method}  & \multicolumn{6}{c}{HDR-NeRF~\cite{hdr-nerf} Real Scenes}                    & \multicolumn{6}{c}{HDR-Plenoxels~\cite{hdr-plenoxels} Real Scenes} \\
\cmidrule(lr){2-7}\cmidrule(lr){8-13}        
&      \multicolumn{3}{c}{LDR-OE ($t_1,t_3,t_5$)} & \multicolumn{3}{c}{LDR-NE ($t_2,t_4$)} & \multicolumn{3}{c}{LDR-OE ($t_1,t_3,t_5$)} & \multicolumn{3}{c}{LDR-NE ($t_2,t_4$)} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}    
&      PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ \\
\midrule       
HDR-NeRF~\cite{hdr-nerf}    & 31.63
&0.948&0.069&31.43&0.943&0.069& - & -&-&-&-&-  \\
% HDR-NeRF~\cite{hdr-nerf} $\dag$     &   31.95    &   0.951    &     0.066  &    31.75   &    0.950   &    0.067   &       &       &       &       &       &  \\
HDR-GS~\cite{hdr-gs} $\dag$ &  33.56    & 0.964   &  0.024     &   31.18    &  0.960     &    0.027   &   30.18    &    0.943   &   0.044    &    27.63 &  0.916& 0.056    \\
\textbf{Ours (3DGS)} &        34.18    & 0.965      &  0.019     &   32.63    &   0.962    &   0.021    &  30.99     &   0.947    &    0.041   &     28.08&0.923&0.050\\
HDR-Scaffold-GS~\cite{scaf-gs} $*$  & 34.09   &   0.967    &  0.016     &    31.88   &    0.964   &   0.019    &    31.05   &   0.944    &   0.045    &   28.13    &   0.916    &   0.059    \\
\textbf{Ours (Scaffold-GS)}   &  \textbf{35.37} & \textbf{0.972} &  \textbf{0.014} &  \textbf{33.68}  &    \textbf{0.969}   &   \textbf{0.016}   &  \textbf{32.24}    &   \textbf{0.954}    &    \textbf{0.031}   &   \textbf{28.98}    &  \textbf{0.932}     & \textbf{0.041} \\   
    \bottomrule
    \end{tabular}}
       \begin{tablenotes}
        \footnotesize
        \item $\dag$ We re-implement HDR-GS~\cite{hdr-gs} under Exp-1 setting for fair comparison.
        \item $*$ We replace the scene representation in HDR-GS from 3DGS~\cite{3dgs} to Scaffold-GS~\cite{scaf-gs} to establish a baseline for our method utilizing Scaffold-GS.
     \end{tablenotes}
  \label{tab:sup_table1}%
\end{table*}%

==> tables/sup_table2.tex <==
\begin{table*}[h]
  \centering
  % \vspace{-360mm}
  \caption{Quantitative comparisons on HDR-NeRF~\cite{hdr-nerf} synthetic datasets. Metrics are averaged over all scenes. LDR-OE and LDR-NE denote the LDR results with exposure $\{t_1,t_3,t_5\}$ and $\{t_2,t_4\}$, respectively. HDR denotes the HDR results. The training setting is Exp-1.}
  \vspace{-2mm}
  \resizebox{0.85\textwidth}{!}{
    \begin{tabular}{c|ccccccccc}
    \toprule
\multirow{2}[4]{*}{Method}    &      \multicolumn{3}{c}{LDR-OE ($t_1,t_3,t_5$)} & \multicolumn{3}{c}{LDR-NE ($t_2,t_4$)} & \multicolumn{3}{c}{HDR}  \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10} 
&      PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$ & PSNR$\uparrow$  & SSIM$\uparrow$  & LPIPS$\downarrow$  \\
   
\midrule     
HDR-NeRF~\cite{hdr-nerf}     & 39.07 &0.973& 0.026 &37.53& 0.966 &0.024 &36.40 &0.936&0.018  \\
% HDR-NeRF~\cite{hdr-nerf} $\dag$ &       39.56 & 0.971 & 0.021 & 38.82 & 0.970 & 0.023 & 37.13 & 0.957 & 0.025 \\
HDR-GS~\cite{hdr-gs} $\dag$ &   39.35	&	0.977	&0.012& 38.01& 0.976	&	0.013     &  22.58&0.840	&0.075  \\
\textbf{Ours (3DGS)}  & 41.51	&0.984	&0.008&41.03 &0.983	&0.009 &37.41&0.969&	0.017     \\
HDR-Scaffold-GS~\cite{scaf-gs} $*$ &  42.21 &	0.986	&0.005	&40.44 & 0.986	&0.006  & 26.11 & 0.915&0.062  \\
\textbf{Ours (Scaffold-GS)} & \textbf{42.94}	&\textbf{0.988} &\textbf{0.004}&	\textbf{42.02}& \textbf{0.988}	&	\textbf{0.005} & \textbf{38.60}&\textbf{0.975}	&\textbf{0.011} \\   
    \bottomrule
    \end{tabular}}
       \begin{tablenotes}
        \footnotesize
        \item $\dag$ We re-implement HDR-GS~\cite{hdr-gs} under Exp-1 setting for fair comparison. Note that the authors of HDR-GS utilize HDR ground truth (GT) for supervision during training on synthetic datasets, whereas our re-implementation does not include this supervision.
        \item $*$ We replace the scene representation in HDR-GS from 3DGS~\cite{3dgs} to Scaffold-GS~\cite{scaf-gs} to establish a baseline for our method utilizing Scaffold-GS.
     \end{tablenotes}
  \label{tab:sup_table2}%
\end{table*}%


